Energy Structure of Optimal Positional Strategies in Mean Payoff Games

This note studies structural aspects concerning Optimal Positional Strategies (OPSs) in Mean Payoff Games (MPGs), it is a contribution to understanding the relationship between OPSs in MPGs and Small Energy-Progress Measures (SEPMs) in reweighted Energy Games (EGs). Firstly, it is observed that the space of all OPSs, $\texttt{opt}_{\Gamma}\Sigma^M_0$, admits a unique complete decomposition in terms of so-called extremal-SEPM{s} in reweighted EG{s}; this points out what we called the "Energy-Lattice $\mathcal{X}^*_{\Gamma}$ of $\texttt{opt}_{\Gamma}\Sigma^M_0$". Secondly, it is offered a pseudo-polynomial total-time recursive procedure for enumerating (w/o repetitions) all the elements of $\mathcal{X}^*_{\Gamma}$, and for computing the corresponding partitioning of $\texttt{opt}_{\Gamma}\Sigma^M_0$. It is observed that the corresponding recursion tree defines an additional lattice $\mathcal{B}^*_{\Gamma}$, whose elements are certain subgames $\Gamma'\subseteq \Gamma$ that we call basic subgames. The extremal-SEPMs of a given \MPG $\Gamma$ coincide with the least-SEPMs of the basic subgames of $\Gamma$; so, $\mathcal{X}^*_{\Gamma}$ is the energy-lattice comprising all and only the least-SEPMs of the \emph{basic} subgames of $\Gamma$. The complexity of the proposed enumeration for both $\mathcal{B}^*_{\Gamma}$ and $\mathcal{X}^*_{\Gamma}$ is $O(|V|^3|E|W |\mathcal{B}^*_{\Gamma}|)$ total time and $O(|V||E|)+\Theta\big(|E| \mathcal{B}^*_{\Gamma}|\big)$ working space. Finally, it is constructed an \MPG $\Gamma$ for which $|\mathcal{B}^*_{\Gamma}| > |\mathcal{X}^*_\Gamma|$, this proves that $\mathcal{B}^*_{\Gamma}$ and $\mathcal{X}^*_\Gamma$ are not isomorphic.

==> Faster.Algo-Sect3-On-Truncated-Total-Payoff.tex <==
\section{On Truncated-Total-Payoff Games, Optimal Strategies in \MPG{s}, and Energy Games}
In \cite{ZwickPaterson:1996}, another variant of payoff game model was considered.
For any $k\geq 0$, the two players play a game for exactly $k$ steps constructing a path of length $k$.
The \emph{total} weight of the constructed path is the outcome of the game,
and the length $k$ of the game is known in advance to both players.
We refer to this model as \emph{k-Truncated-Total-Payoff Game (k-TTPG)}.
Clearly, the values of a $k$-truncated-game can be easily computed in time $O(k|E|)$,
for any $k>0$, by means of the following recursive relation:
\[\displaystyle
\nu_k(u) = \left\{
	\begin{array}{ll}
		\max_{(u,v)\in E} \big( w(u,v) + \nu_{k-1}(v) \big), & \text{ if } u \in V_0 \\
		\min_{(u,v)\in E} \big( w(u,v) + \nu_{k-1}(v) \big), & \text{ if } u \in V_1 \\
	\end{array}
\right.
\] where $\nu_0(u) = 0$ for every $u\in V$.

Unfortunately, as already observed in~\cite{ZwickPaterson:1996},
optimal moves in the truncated games may not conform to positional optimal strategies.
In order to clarify this intuition, we propose the example depicted in Figure \ref{fig:counterexample}.

\begin{figure}[th]
\centering
\begin{tikzpicture}[arrows=->, scale=.75, node distance=.5 and 1]
    \node[node, thick, color=red] (v1) {$v_1$};
    \node[node, thick, color=blue, fill=blue!20, below right =of v1] (v2) {$v_2$};
    \node[node, thick, color=blue, fill=blue!20, below = of v2, yshift=-2ex] (v3) {$v_3$};
    \node[node, thick, color=blue, fill=blue!20, right = of v2, yshift=-5ex] (u) {$u$};
    \node[node, thick, color=red, below left = of v3] (v4) {$v_4$};
    \node[node, thick, color=red, above left =of v4] (v5) {$v_5$};
    \node[node, thick, color=red, above = of v5, yshift=2ex] (v6) {$v_6$};
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \draw[] (v1) to node[xshift=1ex, yshift=1ex, scale=.8] {$-10$} (v2);
    \draw[] (v2) to node[xshift=-1ex, yshift=0ex, scale=.8] {$0$} (v3);
    \draw[] (v2) to node[xshift=0ex, yshift=1ex, scale=.8] {$+1$} (u);
    \draw[] (u) to node[xshift=0ex, yshift=-1ex, scale=.8] {$0$} (v3);
    \draw[] (v3) to node[xshift=0ex, yshift=-1ex, scale=.8] {$0$} (v4);
    \draw[] (v4) to node[xshift=0ex, yshift=-1ex, scale=.8] {$0$} (v5);
    \draw[] (v4) to node[xshift=1ex, yshift=1ex, scale=.8] {$-1$} (v6);
    \draw[] (v5) to node[xshift=-1ex, yshift=0ex, scale=.8] {$0$} (v6);
    \draw[] (v6) to node[xshift=-1.5ex, yshift=1ex, scale=.8] {$+10$} (v1);
\end{tikzpicture}
\caption{An arena in which the optimal strategies of the corresponding TTPG are not positional.}%%
\label{fig:counterexample}
\end{figure}

We now argue that optimal moves in the truncated game may depend on the particular
value of $k$ that a player find himself moving, as well as on the history of the opposite player.
Therefore, depending on how many moves remains to play and on the history of the opposite player,
the players may be forced to move the pebble suboptimally with respect to the traditional game.
Indeed, the $k$-truncated-game model is not memoryless, \ie generally, there is no positional optimal strategy.
Notice that suboptimality can last for the entire truncated game's duration,
\ie a player can be forced to always deviate from his positional optimal strategy.
Even though $k$-truncated-games provide good approximations of optimal values,
their paths may deviate from the underlying positional optimal strategy in a very strong sense.
This interesting and surprising behavior unveils the difficulty of designing a procedure
for the reconstruction of positional optimal strategies by means of $k$-truncated-games,
without increasing the complexity of computing the optimal values.
To overcome this, we propose a novel model of truncated games called
\emph{Min-$k$-Truncated-Total-Payoff Games (Min-$k$-TTPGs)}.
\begin{Def}[Min-$k$-TTPG]\label{def:newgame}
For any $k\geq 0$, the two players move the pebble on $\Gamma$ as in the $k$-Truncated-Game, but, Player~$1$ has an additional power:
before each pebble's move, Player~$1$ may decrease the number of the remaining moves, arbitrarily.
Specifically, suppose that the pebble is at vertex $v\in V_{p}$ for some $p\in\{0,1\}$,
if the play has $r$ remaining moves, then, before Player~$p$ moves the pebble from $v$ to some of its neighbors,
Player~$1$ updates $r$ to $r'$ for some $0\leq r'\leq r$.
Naturally, if $r'=0$ the game is over;
otherwise, $r'>0$ and Player~$p$ moves the pebble and the next turn will have $r'-1$ remaining moves.
The game continues so on until there is no remaining move (\ie $r=0$).
The value of the game when starting at $v\in V$ is denoted by $\nu'_k(v)$.
\end{Def}

In a Min-$k$-TTPG, Player~$1$ may decide to consume all moves at disposal immediately,
\ie before the pebble moves for the first time, thus attaining zero payoff. This implies the following.
\begin{Prop} It holds that $\nu'_k(v)\leq 0$ for every $v\in V$ and $k\geq 0$. \end{Prop}
The values of a Min-$k$-TTPG satisfy the following recursive relation, which is obtained by slightly adjusting that of $k$-TTPGs.
\begin{Prop}\label{prop:recursive}
It holds $\nu'_0(v)=0$ for every $v\in V$. Moreover, for any $k>0$, the following recursive relation holds:
\[\displaystyle
	\nu'_k(u) = \left\{
		\begin{array}{ll}
			\min\Big (\nu'_{k-1}(u), \max_{(u,v)\in E} \big(w(u,v) + \nu'_{k-1}(v) \big)\Big ), & \text{ if } u \in V_0 \\
			\min\Big (\nu'_{k-1}(u), \min_{(u,v)\in E} \big(w(u,v) + \nu'_{k-1}(v) \big)\Big ), & \text{ if } u \in V_1 \\
		\end{array}
	\right.
\]
\end{Prop}
Notice, from Proposition~\ref{prop:recursive}, that having more moves is a benefit only for Player~1.
\begin{Prop}\label{prop:monotonicity}
For every $k\geq 1$ and every $u\in V$, it holds that $\nu'_{k-1}(u) \geq \nu'_{k}(u)$.
\end{Prop}
Next, we observe a sort of regularity condition for Min-$k$-TTPGs.
Recall that when the game starts at some $v\in V$, Player~1 has to choose whether
to stay at that vertex and decreasing number of moves available $r$ -- even if $v\in V_0$ --
or whether to let the pebble moves to a new vertex through some arc going out of $v$:
the next proposition shown that if the optimal behaviour of Player~1, when starting at $v$, is that to decrease $r$ by some amount,
then the choice of completely reset $r$ to zero is optimal as well.
Stated otherwise, it is never the case that Player~1 needs to
stop moving the pebble for a bit of rounds and afterwhile to start moving it. This is formally shown below.
\begin{Prop}\label{prop:stop_is_gameover}
For any $k\geq 1$, the following holds:
\begin{itemize}
\item If $u\in V_0$ and $\nu'_{k-1}(u) < \max_{(u,v)\in E} \big(w(u,v) + \nu'_{k-1}(v) \big)$, then $\nu'_k(u)=0$;
\item If $u\in V_1$ and $\nu'_{k-1}(u) < \min_{(u,v)\in E} \big(w(u,v) + \nu'_{k-1}(v) \big)$, then $\nu'_k(u)=0$;
\end{itemize}
\end{Prop}
\begin{proof}
Assume $u\in V_0$. The proof goes by induction on $k\geq 1$.

\emph{Base Case.}
If $k=1$, then $\nu'_{k-1}(v)=\nu'_{0}(v)=0$ holds for every $v\in V$.
If the inequality $\nu'_{k-1}(u) < \max_{(u,v)\in E} \big\{w(u,v) + \nu'_{k-1}(v) \big\}$ holds,
then, by Proposition~\ref{prop:recursive}, $\nu'_k(u) = \nu'_{k-1}(u) = 0$.

\emph{Inductive Step.}
Let us assume the thesis to be true up to $k-1$, and let us prove it for $k\geq 2$.
Assume $\nu'_{k-1}(u) < \max_{(u,v)\in E} \big\{w(u,v) + \nu'_{k-1}(v) \big\}$.
Then, we argue that the following holds:
\[
	\nu'_{k-1}(u) = \nu'_{k-2}(u) < \max_{(u,v)\in E} \big(w(u,v) + \nu'_{k-2}(v) \big) \tag{$*$}
\]
In fact, by Proposition~\ref{prop:recursive}, since $u\in V_0$, it must be that either $(*)$ holds or that the following holds:
\[
	\nu'_{k-1}(u) = \max_{(u,v)\in E} \big(w(u,v) + \nu'_{k-2}(v) \big) \tag{$**$}
\]
However, $(**)$ is not possible, since otherwise we get the following inequality:
\[
	\max_{(u,v)\in E} \big(w(u,v) + \nu'_{k-2}(v) \big) = \nu'_{k-1}(u) < \max_{(u,v)\in E} \big(w(u,v) + \nu'_{k-1}(v) \big),
\]
picking $\hat{v}\triangleq\arg\max_{\{v\in V\mid (u,v)\in E\}} \big(w(u,v) + \nu'_{k-1}(v)\big)$,
one obtains:
\[
	w(u,\hat{v}) + \nu'_{k-2}(\hat{v}) \leq \max_{(u,v)\in E} \big(w(u,v) + \nu'_{k-2}(v) \big) =
	\nu'_{k-1}(u) < w(u,\hat{v}) + \nu'_{k-1}(\hat{v}),
\]
that implies, in particular, $\nu'_{k-2}(\hat{v}) < \nu'_{k-1}(\hat{v})$, which is absurd by Proposition~\ref{prop:monotonicity}.

Therefore, ($*$) must hold instead of ($**$).

At this point, since $\nu'_{k-2}(u) < \max_{(u,v)\in E} \big( w(u,v) + \nu'_{k-2}(v) \big)$ holds by ($*$),
then, by induction hypothesis, $\nu'_{k-1}(u)=0$.
On the other hand, since $\nu'_{k-1}(u) < \max_{(u,v)\in E} \big( w(u,v) + \nu'_{k-1}(v) \big)$ by assumption,
then $\nu'_k(u)=\nu'_{k-1}(u)$ by Proposition~\ref{prop:recursive}. Therefore, $\nu'_k(u)=\nu'_{k-1}(u)=0$.

A symmetric argument works when $u\in V_1$.
\end{proof}

\begin{Prop}\label{prop:value_minus_inf}
Let $\Gamma=(V,E,w,\langle V_0, V_1\rangle)$ be an arena and let $k\in\N$.

The following holds for every $v\in\W_1$:
\[\nu'_k(v)\leq -\left\lfloor \frac{k}{|\W_1|} \right\rfloor + \big(|\W_1|-1\big)W.\]
Therefore, $\lim_{k\rightarrow+\infty}\nu'_{k}(v) = -\infty$ for every $v\in\W_1$.
\end{Prop}
\begin{proof} Let $v\in\W_1$. Then, there is a \emph{positional} strategy $\sigma_1\in\Sigma^M_{1}$
such that $\val{\sigma_1}{v}< 0$. Suppose that, in the Min-$k$-TTPG played on $\Gamma$,
Player~1 adopts the following strategy:

-- never decreases the number $r$ of remaining moves, and move the pebble according to $\sigma_1$.

Since $\val{\sigma_1}{v}< 0$, all cycles that are reachable from $v$ in $G^{\Gamma}_{\sigma_1}$ have a negative total weight.
Therefore, every $|\W_1|$ moves of the pebble, at least one such a negative cycle $C$ is formed, and $w(C) \leq - 1$.
Since Player~$1$ never decreases the number $r$ of the remaining moves, and the game starts with $k$ available moves,
then the number of negative cycles that are visited during the whole play is at least $\lfloor k/|\W_1|\rfloor$.
Moreover, the number of arcs traversed during the game that do not belong to any of those negative cycles is at most $|\W_1|-1$,
because the sequence of such arcs forms an acyclic path in $\W_1$; therefore, the total weight of all those arcs that do not
belong to the above mentioned family of negative cycles is at most $(|\W_1|-1)W$.
These facts imply altogether that the total weight $w(p)$ of \emph{any} path $p$,
that is formed during such a play, is at most:
\[
	w(p)\leq -\left\lfloor {k}/{|\W_1|}\right\rfloor + (|\W_1|-1)W.
\]
Then, $\nu'_k$ satisfies the same upper-bound for every starting position $v\in\W_1$.

Moreover, this implies that,
as the number of initially available moves $k$ increases (\ie as $k\rightarrow +\infty$),
$\nu'_k(v)$ is not bounded from below, for any $v\in \W_1$.
Therefore, $\lim_{k\rightarrow+\infty}\nu'_{k}(v) = -\infty$.
\end{proof}


\begin{Lem}\label{lem:convergenza}
Let $\Gamma=(V,E,w,\langle V_0, V_1\rangle)$ be an arena.
Let $\W_0$ be the winning region of Player~0 in the \EG played on $\Gamma$.
For any $k\in\N$, let $\{\nu'_k(v)\}_{v\in V}$ be the values of the Min-$k$-TTPG on $\Gamma$.

Then, the following holds:
\begin{enumerate}
\item $-(|\W_0|-1)W\leq \nu'_k(v)\leq 0$ holds for every $k\geq 0$ and $v\in \W_0$;

\item For every $k\in\N$, there exists some $1\leq \hat{k}\leq (|\W_0|-1)|\W_0|W+1$ such that
$\nu'_{k+\hat{k}}(v) = \nu'_{k+\hat{k}-1}(v)$ holds for every $v\in \W_0$.
\end{enumerate}
\end{Lem}
\begin{proof}
Let $v\in \W_0$. Then, there exists a (positional) strategy $\sigma_0\in\Sigma^M_{0}$
such that $\val{\sigma_0}{v}\geq 0$. Suppose that Player~$0$ adopts $\sigma_0$ in the Min-$k$-TTPG played on $\Gamma$.
Since $\val{\sigma_0}{v}\geq 0$, then $G^{\Gamma}_{\sigma_0}$ contains \emph{no} negative cycle that is reachable from $v$.
Therefore, the total-payoff value $\nu'_k(v)$ of the corresponding Min-$k$-TTPG is at least $-(|\W_0|-1)W$,
which is the total weight of the most negative (possible) acyclic path that starts from $v$ in $G^{\Gamma}_{\sigma_0}$.
Hence, for every $k\geq 0$, $-(|\W_0|-1)W\leq \nu'_k(v)\leq 0$ holds for every $v\in \W_0$.

Let us fix $k\in\N$. Consider the values $\nu'_j(v)$ for $v\in \W_0$, for increasing $j=k+1, k+2, \cdots$.
For each $j$, either the fixpoint condition $\nu'_{j}(v) = \nu'_{j-1}(v)$ holds for every $v\in \W_0$,
or there exists $\hat{v}\in \W_0$ such that $\nu'_j(\hat{v})<\nu'_{j-1}(\hat{v})$ (by Proposition~\ref{prop:monotonicity}).
Therefore, since $-(|\W_0|-1)W\leq \nu'_j(v)\leq 0$ holds for every $v\in\W_0$ and $j\in\N$,
there must be some $1\leq \hat{k}\leq (|\W_0|-1)|\W_0| W+1$
such that $\nu'_{k+\hat{k}}(v) = \nu'_{k+\hat{k}-1}(v)$ holds for every $v\in \W_0$.
\end{proof}

\begin{Lem}\label{lem:nu_geq_f}
Let $\Gamma=(V, E, w, V_0\cup V_1)$ be an arena. Let $f^*$ be the least-SEPM of the \EG $\Gamma$,
and let $\W_0$ be the winning region of Player~0 in the \EG $\Gamma$.

For any $k\in\N$, let $\{\nu'_k(v)\}_{v\in V}$ be the values of the Min-$k$-TTPG played on $\Gamma$.

Then, $\nu'_{k}(v)\geq -f^*(v)$ holds for every $v\in \W_0$ and $k\in \N$.
\end{Lem}
\begin{proof}
Let $\sigma^*_0\in\Sigma^M_0$ be a (positional) strategy compatible with $f^*$ in $\Gamma$.
Let $j\in\N$, arbitrarily. Let $p=v_1v_2\cdots v_{j}$ be any path (not necessarily acyclic) in $G^{\Gamma}_{\sigma^*_0}$ of length $j$.
Since $\sigma^*_0$ is compatible with $f^*$ in $\Gamma$, then $f^*(v_1)+\sum_{i=1}^{j-1} w(v_i, v_i+1) \geq 0$;
in fact, the following holds:
\begin{align*}
f^*(v_1)  &  \geq f^*(v_2) - w(v_1,v_2) & \text{[$(v_1,v_2)\in E$ is compatible with $f^*$]} \\
	  &  \geq f^*(v_3) - w(v_1,v_2) -w(v_2,v_3) & \text{[$(v_2,v_3)\in E$ is compatible with $f^*$]} \\
	  &  \cdots & \text{[by induction ...]} \\
   	  &  \geq f^*(v_j) - \sum_{i=1}^{j-1}w(v_i, v_i+1) & \text{[$(v_{j-1},v_j)\in E$ is compatible with $f^*$]}
\end{align*}
Therefore, $f^*(v_1) + \sum_{i=1}^{j-1}w(v_i, v_i+1) \geq f^*(v_j) \geq 0$.

This proves that $w(p)\triangleq\sum_{i=1}^{j-1}w(v_i, v_i+1) \geq -f^*(v_1)$ holds for every (not necessarily acyclic)
path $p=v_1v_2\cdots v_{j}$ in $G^{\Gamma}_{\sigma^*_0}$ of any length $j\in\N$.
Next, for any $k\in\N$, assume that Player~0 adopts $\sigma^*_0$ in the Min-$k$-TTPG played on $\Gamma$,
starting from some $v\in \W_0$. Let $p$ be any (not necessarily acyclic) path in $G^{\Gamma}_{\sigma^*_0}$
that is formed during such a Min-$k$-TTPG match, no matter how Player~1 decides to play.
Since $p$ is a path in $G^{\Gamma}_{\sigma^*_0}$, then $w(p)\geq -f^*(v)$ holds, as shown above.
Therefore, $\nu'_{k}(v)\geq -f^*(v)$ holds for every $v\in \W_0$ and $k\in \N$.
\end{proof}

\begin{Thm}\label{prop:MinkTTPGs_are_SEPMs}
Let $\Gamma=(V, E, w, V_0\cup V_1)$ be an arena. Let $f^*$ be the least-SEPM of the \EG $\Gamma$.

For any $k\geq 0$, let $\{\nu'_k(v)\}_{v\in V}$ be the values of the Min-$k$-TTPG played on $\Gamma$.
Moreover, let: \[k'\triangleq \big( |V|W-2W+1 \big)|\W_1|+(|\W_0|-1)|\W_0|W+3.\]

Then, for every $\kappa\geq k'$ the following holds:
\[
	\nu'_{\kappa}(v) = -f^*(v), \text{ for every } v\in \W_0.
\]
Therefore, $\lim_{k\rightarrow+\infty}\nu'_{k}(v) = - f^*(v)$ for every $v\in V$.
\end{Thm}
\begin{proof}
By Lemma~\ref{lem:nu_geq_f}, we know that $\nu'_k(u)\geq -f^*(u)$ holds for every $k\in\N$ and $u\in \W_0$.
It is thus sufficient to prove that $\nu'_k(u)\leq -f^*(u)$ holds for every $u\in \W_0$ and for every sufficiently large $k$.
In order to do this, let us introduce the following function, for every $u\in V$:
\[
	f^{\nu'_k}(u) \triangleq \left\{
	\begin{array}{ll}
		-\nu'_k(u), & \text{ if } \nu'_k(u)\geq -(|\W_0|-1)W \\
		\top, 	 & \text{ if }	\nu'_k(u) < -(|\W_0|-1)W
	\end{array}
	\right.
\]
We now argue that $f^{\nu'_k}$ is a SEPM of the \EG $\Gamma$, when $k$ is sufficiently large.

To begin, notice that the following holds for every $u\in V$ and for every $k\in\N_0$:
\begin{align*}
	\nu'_{k}(u) & = \left\{
	\begin{array}{ll}
		\min\Big (\nu'_{k-1}(u), \max_{(u,v)\in E} \big(w(u,v) + \nu'_{k-1}(v) \big)\Big ), & \text{ if } u \in V_0 \\
		\min\Big (\nu'_{k-1}(u), \min_{(u,v)\in E} \big(w(u,v) + \nu'_{k-1}(v) \big)\Big ), & \text{ if } u \in V_1 \\
	\end{array}
	\right. & \text{[by Prop.~\ref{prop:recursive}]}
\end{align*}
By Item~2 of Lemma~\ref{lem:convergenza}, for every $v\in\W_0$ and for some $k\in\N$, we know that $\nu'_{k-1}(v)=\nu'_{k}(v)$.
To proceed with the proof, at this point, we would substitute $\nu'_{k-1}$ with $\nu'_{k}$ in the recursive equation above.
However notice that, in the terms
$\max_{(u,v)\in E}\big(w(u,v)+\nu'_{k-1}(v)\big)$ and $\min_{(u,v)\in E}\big(w(u,v)+\nu'_{k-1}(v)\big)$,
one needs to take into account the values $\nu'_{k-1}(v)$ \emph{also} when $v\in\W_1$
(for which $\nu'_{k-1}(v)=\nu'_{k}(v)$ may not hold, generally). Still, we know the following two facts.
By Proposition~\ref{prop:value_minus_inf}, it holds
$\nu'_{k-1}(v)\leq -\left\lfloor{(k-1)}/{|\W_1|}\right\rfloor + (|\W_1|-1)W$ for every $v\in \W_1$ and $k\in\N_0$.
On the other hand, by Item~1 of Lemma~\ref{lem:convergenza},
we know that $\nu'_{k-1}(v)\geq -(|\W_0|-1)W$ holds for every $k\in\N_0$ when $v\in \W_0$.

Therefore, let us now seek for some $k\in\N$ such that the following inequality holds:
\[	-\lfloor (k-1)/|\W_1| \rfloor + (|\W_1|-1)W < -(|\W_0|-1)W \tag{$*$}\]
That is to say, let us pick some $k>k_0$, where:
\[k_0\triangleq \big( |V|W-2W+1 \big) |\W_1|+1, \tag{$**$}\]
Also, at this point, it is worthwhile to introduce the following notation for every $S\subseteq V$, $j\in\N$, and every $u\in V_0$:
\[\max (S,u,j)\triangleq \max_{v\in S:(u,v)\in E}\big(w(u,v)+\nu'_{j}(v)\big),\]
and, similarly, for every $S\subseteq V$, $j\in\N$, \emph{and} $u\in V_1$, $\min (S,u,j)\triangleq
	\min_{v\in S:(u,v)\in E}\big(w(u,v)+\nu'_{j}(v)\big)$.

Then, we argue that the following holds for every $u\in V_0\cap\W_0$ and any $k>k_0$ ($**$):
\[
	\max (V,u,k-1) = \max (\W_0,u,k-1). \tag{$\star_{\max}$}
\]
Indeed, since $u\in\W_0$, then there is \emph{at least one} $\hat{v}\in\W_0$ such that $(u,\hat{v})\in E$, and recall that
$\nu'_{k-1}(\hat{v})+w(u,\hat{v})\geq -(|\W_0|-1)W-W$ holds on $\hat{v}$ by Item~1 of Lemma~\ref{lem:convergenza}.
When $k>k_0$ ($**$), then ($*$) holds, therefore:
\begin{align*}
\max(\W_1,u,k-1) &  \leq -\left\lfloor \frac{k-1}{|\W_1|}
			\right\rfloor + (|\W_1|-1)W - W & \text{[by Prop.~\ref{prop:value_minus_inf}]} \\
		& <  -(|\W_0|-1)W-W & \text{[by ($*$)]}\\
		& \leq \nu'_{k-1}(\hat{v})+w(u,\hat{v}) & \text{[by $\hat{v}\in\W_0$ and Item~1 of Lemma~\ref{lem:convergenza}]} \\
		& \leq \max (\W_0,u,k-1) & \text{[by $\hat{v}\in\W_0$]}
\end{align*}

Hence, the following holds for every $u\in\W_0$ and for every $k>k_0$ ($**$):
\begin{align*}
\max (V,u,k-1)  & = \max\big(\max(\W_0,u,k-1), \max(\W_1,u,k-1)\big) & \text{[by $\W_0\cup\W_1=V$]} \\
		& = \max(\W_0,u,k-1) & \text{[by $\max(\W_1,u,k-1) < \max(\W_0,u,k-1)$]}
\end{align*}
This proves ($\star_{\max}$).

Also notice that the following holds as well for every $u\in V_1\cap\W_0$ and $k\in\N$:
\[\min(V,u,k-1) = \min(\W_0, u, k-1)\tag{$\star_{\min}$}\]
Indeed, when $u\in V_1\cap\W_0$,
	there is \emph{no} $\hat{v}\in\W_1$ such that $(u,\hat{v})\in E$, so that
$\{(u,v)\in E\}=\{(u,v)\in E\mid v\in \W_0\}$. This proves ($\star_{\min}$).

Next, we proceed as follows. Let us fix some $k>k_0$ ($**$).
By Item~2 of Lemma~\ref{lem:convergenza}, for every $u\in\W_0$ there exists some
$1\leq \hat{k}\leq (|\W_0|-1)|\W_0|W+1$ such that $\nu'_{k+\hat{k}}(u)=\nu'_{k+\hat{k}-1}(u)$.
Let $k'\triangleq k+\hat{k}$.
Then, the following holds for every $u\in\W_0$:
\begin{align*}
	\nu'_{k'}(u) & = \left\{
	\begin{array}{ll}
		\min\Big (\nu'_{k'-1}(u), \max(V,u,k'-1)\Big), & \text{ if } u \in V_0 \\
		\min\Big (\nu'_{k'-1}(u), \min(V,u,k'-1)\Big), & \text{ if } u \in V_1 \\
	\end{array}
	\right. & \text{[by Prop.~\ref{prop:recursive}]} \\
	& = \left\{
	\begin{array}{ll}
	\min\Big (\nu'_{k'-1}(u), \max(\W_0,u,k'-1)\Big), & \text{ if } u \in V_0 \\
	\min\Big (\nu'_{k'-1}(u), \min(\W_0,u,k'-1)\Big), & \text{ if } u \in V_1 \\
	\end{array}
	\right. & \text{[by ($**$), $\star_{\max}$ and $\star_{\min}$]} \\
	& = \left\{
	\begin{array}{ll}
	\min\Big (\nu'_{k'}(u), \max(\W_0,u,k')\Big), & \text{ if } u \in V_0 \\
	\min\Big (\nu'_{k'}(u), \min(\W_0,u,k')\Big), & \text{ if } u \in V_1 \\
	\end{array}
	\right. & \text{[by Item~2 of Lemma~\ref{lem:convergenza}]} \\
	& = \left\{
	\begin{array}{ll}
	\min\Big (\nu'_{k'}(u), \max(\W_0,u,k')\Big), & \text{ if } u \in V_0 \\
	\min\Big (\nu'_{k'}(u), \min(V,u,k')\Big), & \text{ if } u \in V_1 \\
	\end{array}
	\right. & \text{[by ($**$) and $\star_{\min}$]}
\end{align*}
Therefore, the following holds for every $u\in\W_0$:
\begin{align*}
	\nu'_{k'}(u) \leq
	\left\{
	\begin{array}{ll}
	 \max(\W_0,u,k'), & \text{ if } u \in V_0 \\
	 \min(V,u,k'), & \text{ if } u \in V_1 \\
	\end{array}
	\right.
\end{align*}
Multiplying both sides by $-1$, and substituting $-\max x$/$\min -x$, and $-\min x$/$\max -x$, for $u\in\W_0$:
\begin{align*}
	-\nu'_{k'}(u) \geq
	\left\{
	\begin{array}{ll}
	 \min_{v\in\W_0 : (u,v)\in E} \big( -\nu'_{k'}(v) - w(u,v) \big), & \text{ if } u \in V_0 \\
	 \max_{(u,v)\in E} \big( -\nu'_{k'}(v) - w(u,v) \big), & \text{ if } u \in V_1 \\
	\end{array}
	\right. \tag{$\checkmark$}
\end{align*}
We are almost done, further notice that the following two facts hold for $k'$:

($\dagger$) when $u\in\W_0$, it holds $f^{\nu'_{k'}}(u)=-\nu'_{k'}(u)$:
in fact, since $u\in\W_0$, then by Item~1 of Lemma~\ref{lem:convergenza},
it holds $\nu'_{k'}(u)\geq -(|\W_0|-1)W$.

($\ddagger$) when $u\in\W_1$, it holds $f^{\nu'_{k'}}(u)=\top$:
in fact, since $k'$ satisfies ($**$), then ($*$) holds; therefore,
by Proposition~\ref{prop:value_minus_inf}, it holds
$\nu'_{k'}(u)\leq -\left\lfloor{k'}/{|\W_1|}\right\rfloor + (|\W_1|-1)W < -(|\W_0|-1)W$.

At this point, we've finally come in the position to check that $f^{\nu'_{k'}}$ is a SEPM for the \EG $\Gamma$.

In fact, the following holds for $k'$:

-- if $u\in \W_1$, then:
\[
	f^{\nu'_{k'}}(u)\overset{\text{[by ($\ddagger$)]}}{=}
			\top \succeq f^{\nu'_{k'}}(v) \ominus w(u,v), \text{ for every } (u,v)\in E.
\]

-- if $u\in V_0\cap\W_0$, then:
	\begin{align*}
	f^{\nu'_{k'}}(u)  \overset{\text{[by ($\dagger$)]}}{=} -\nu'_{k'}(u) &
						\overset{\text{[by ($\checkmark$)]}}{\succeq} -\nu'_{k'}(v) \ominus w(u,v),
								 \text{ for \emph{some} } (u, v)\in E \text{ such that } v\in\W_0, \\
		& \overset{\text{[by ($\dagger$)]}}{=} f^{\nu'_{k'}}(v) \ominus w(u,v).
	\end{align*}

-- if $u\in V_1\cap\W_0$, then:
	\begin{align*}
f^{\nu'_{k'}}(u) \overset{\text{[by ($\dagger$)]}}{=}
	-\nu'_{k'}(u) & \overset{\text{[by ($\checkmark$)]}}{\succeq} -\nu'_{k'}(v) \ominus w(u,v),
					\text{ for \emph{all} } (u, v)\in E.\\
				& \overset{\text{[by ($\dagger$)]}}{=} f^{\nu'_{k'}}(v) \ominus w(u,v).
	\end{align*}
Where the last equality holds by ($\dagger$), because when $u\in V_1\cap\W_0$
	there is \emph{no} $v\in\W_1$ such that $(u,v)\in E$;
thus, if $u\in V_1\cap\W_0$ and $(u,v)\in E$, then $f^{\nu'_{k'}}(v)=-\nu'_{k'}(v)$.

This concludes the proof that $f^{\nu'_{k'}}$ is a SEPM for the \EG $\Gamma$.

Since $f^*$ is the \emph{least}-SEPM of the \EG $\Gamma$, then $f^*(v)\preceq f^{\nu'_{k'}}(v)$ holds for every $v\in V$.

Therefore, for $k'\triangleq k+\hat{k}$ as defined above, it holds that:
\[
	- \nu_{k'}(u) = f^{\nu_{k'}}(u) \leq f^*(u), \text{ for every } u\in\W_0.
\]

Since we have shown that $f^*(u)\leq -\nu'_{k'}(u)$ and $-\nu'_{k'}(u)\leq f^*(u)$ holds for every $u\in\W_0$,
then $\nu'_{k'}(u)=-f^*(u)$ holds for every $u\in\W_0$.

We now argue that for every $\kappa\geq k'$ the equality $\nu'_{\kappa}(u)=-f^*(u)$ holds for every $u\in\W_0$.
Indeed, we already know the following three facts:

(1) The equality holds for $\kappa=k'$, as just shown above;

(2) $\nu'_{j-1}(u) \geq \nu'_{j}(u)$ holds for every $j\geq 1$ and every $u\in V$, by Proposition~\ref{prop:monotonicity}.

(3) $\nu'_{j}(u)\geq -f^*(u)$ holds for every $u\in \W_0$ and every $j\in \N$, by Lemma~\ref{lem:nu_geq_f};

These facts together imply that, for every $\kappa\geq k'$ and $u\in\W_0$:
\[ -f^*(u) \overset{\text{[by (1)]}}{=} \nu'_{k'}(u)
		\overset{\text{[by (2)]}}{\geq} \nu'_{\kappa}(u) \overset{\text{[by (3)]}}{\geq} -f^*(u).
\]
This proves that, for every $\kappa\geq k'$, it holds $\nu'_{\kappa}(u)=-f^*(u)$ for every $u\in\W_0$.

The only remaining point concerns the magnitude of $k'$.
We have $k'=k+\hat{k}$, where $k>k_0$ as in ($**$),
and $1\leq \hat{k}\leq (|\W_0|-1)|\W_0|W+1$; therefore:
$k_0 < k' \leq k_0 + (|\W_0|-1)|\W_0|W + 2$.
\end{proof}
Notice that $k'=\Omega\big(|V||\W_1|W \big)$ and $k'=O\big(|V||\W_1|W + |W_0|^2 W\big)$.

